Urban Radiance Field Representation with Deformable Neural Mesh Primitives

Neural Radiance Fields (NeRFs) have achieved great success in the past few years. However, most current methods still require intensive resources due to ray marching-based rendering. To construct urban-level radiance fields efficiently, we design Deformable Neural Mesh Primitive~(DNMP), and propose to parameterize the entire scene with such primitives. The DNMP is a flexible and compact neural variant of classic mesh representation, which enjoys both the efficiency of rasterization-based rendering and the powerful neural representation capability for photo-realistic image synthesis. Specifically, a DNMP consists of a set of connected deformable mesh vertices with paired vertex features to parameterize the geometry and radiance information of a local area. To constrain the degree of freedom for optimization and lower the storage budgets, we enforce the shape of each primitive to be decoded from a relatively low-dimensional latent space. The rendering colors are decoded from the vertex features (interpolated with rasterization) by a view-dependent MLP. The DNMP provides a new paradigm for urban-level scene representation with appealing properties: $(1)$ High-quality rendering. Our method achieves leading performance for novel view synthesis in urban scenarios. $(2)$ Low computational costs. Our representation enables fast rendering (2.07ms/1k pixels) and low peak memory usage (110MB/1k pixels). We also present a lightweight version that can run 33$\times$ faster than vanilla NeRFs, and comparable to the highly-optimized Instant-NGP (0.61 vs 0.71ms/1k pixels). Project page: \href{https://dnmp.github.io/}{https://dnmp.github.io/}.

==> figure/teaser.tex <==
\begin{figure}
 \includegraphics[angle=0,origin=c, width=1\linewidth, trim=0cm 0cm 0cm 0cm, clip]{resource/teaser.pdf}

\end{figure}

==> supple_figure/comparison_kitti.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=1\linewidth, trim=0cm 0cm 0cm 0cm, clip]{supple_resource/comparison_kitti360_supple_v1.pdf}
    \caption{Qualitative comparison of novel view synthesis on KITTI-360 dataset. Cropped patches are scaled to highlight details. Due to the explicit and accurate surface modeling, the proposed method significantly outperforms baseline methods and can effectively recover texture details.}
    \label{fig:comparison_kitti}
\end{figure*}

==> supple_figure/comparison_waymo_supple.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=1\linewidth, trim=0cm 0cm 0cm 0cm, clip]{supple_resource/comparison-waymo-supple-v2.pdf}
    \caption{Qualitative comparison of novel view synthesis on Waymo dataset. Cropped patches are scaled to highlight details. Due to the explicit and accurate surface modeling, the proposed method significantly outperforms baseline methods and can effectively recover texture details.}
    \label{fig:comparison_waymo_supple}
\end{figure*}

==> supple_figure/latent_code.tex <==
\begin{figure}
% \setlength{\abovecaptionskip}
\centering
{
 \includegraphics[width=0.95\linewidth]{supple_resource/latent_code.pdf}
 }
\caption{Optimization of DNMPs. DNMPs can be deformed from 
spherical template meshes into various basic shapes (\emph{e.g.}, plane, pillar, curved surface, \etc), via optimizing the shape latent codes.}
\label{fig:latent_code}
\end{figure}

==> supple_figure/metashape.tex <==
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=1\linewidth, trim=0cm 0cm 0cm 0cm, clip]{supple_resource/metashape.pdf}
    % \vspace{-3ex}
    \caption{Qualitative comparison of novel view synthesis on KITTI-360 dataset with neural rendering using meshes reconstructed from Multi-View Stereo (MVS). Cropped patches are scaled to highlight details. Reconstructed meshes from MVS are incomplete (\emph{e.g.}, the upper part of the car in the cropped patches in the first row) and contain occlusions (\emph{e.g.}, the building in the bottom-right corner of the cropped patches in the second row), leading to blurry and unreal rendering results.}
    \label{fig:metashape}
    % \vspace{-3ex}
\end{figure*}

==> supple_figure/primitive_radius.tex <==
\begin{figure}
% \resizebox{1.0\linewidth}{!}
\centering
{
 \includegraphics[width=0.95\linewidth]{supple_resource/primitive_radius.pdf}
 }
\caption{View synthesis results based on DNMPs of different sizes. Even only based on the DNMP with a dimension of 2 meters,  the synthesized images are still of acceptable quality,    
though the texture details are lost compared to results of 0.5m-DNMPs.
}
\label{fig:primitive_radius}
\end{figure}

==> supple_figure/scannet.tex <==
\begin{figure}[htbp]
\centering
{\includegraphics[width=1.\linewidth]{supple_resource/scannet.pdf}}
\caption{A sample of rendering results on ScanNet dataset.}
\label{fig:scannet}
\end{figure}

==> supple_figure/semantic.tex <==
\begin{figure}
\setlength{\abovecaptionskip}{1ex}
 \includegraphics[width=1\linewidth]{supple_resource/semantic.pdf}
\caption{Novel semantic synthesis.}
\label{fig:semantic}
\end{figure}

==> supple_table/comparison_large_nerfs.tex <==
\begin{table}[htbp]
\centering
\footnotesize
\caption{
Comparison with large-scale NeRFs. The comparison is based on KITTI-360 dataset. 
}
\label{tab:comparison_large}

\setlength{\tabcolsep}{5mm}{
{
\begin{tabular}{l c c c}
\toprule
\multirow{1}{*}{\textbf{Methods}} & \multicolumn{1}{c}{PSNR$\uparrow$} & \multicolumn{1}{c}{SSIM$\uparrow$} & \multicolumn{1}{c}{LPIPS$\downarrow$}\\
\midrule
BungeeNeRF~\cite{xiangli2022bungeenerf} & 22.02 & 0.788 & 0.429 \\ 
Mega-NeRF~\cite{turki2022mega} & 23.15 & 0.826 & 0.326 \\
\midrule
Ours & \textbf{23.41} & \textbf{0.846} & \textbf{0.305} \\  
            
\bottomrule
\end{tabular}
}}
\end{table}

==> supple_table/comparison_mesh.tex <==
\begin{table}[htbp]
\centering
\footnotesize
\caption{
Comparison with neural rendering using meshes reconstructed from Multi-View Stereo (MVS). The comparison is based on KITTI-360 dataset. 
}
\label{tab:comparison_mesh}

\setlength{\tabcolsep}{5mm}{
{
\begin{tabular}{l c c c}
\toprule
\multirow{1}{*}{\textbf{Methods}} & \multicolumn{1}{c}{PSNR$\uparrow$} & \multicolumn{1}{c}{SSIM$\uparrow$} & \multicolumn{1}{c}{LPIPS$\downarrow$}\\
\midrule
MVS~\cite{metashape} & 21.82 & 0.817 & 0.341 \\  
Ours & \textbf{23.41} & \textbf{0.846} & \textbf{0.305} \\  
            
\bottomrule
\end{tabular}
}}
\end{table}

==> supple_table/comparison_mobile.tex <==
\begin{table}[htbp]
\centering
\footnotesize
\caption{
Comparison with MobileNeRF. 
}
\label{tab:comparison_mobile}

\setlength{\tabcolsep}{3mm}{
{
\begin{tabular}{l c c c c}
\toprule
\multicolumn{2}{c}{\textbf{Methods}} & \multicolumn{1}{c}{PSNR$\uparrow$} & \multicolumn{1}{c}{SSIM$\uparrow$} & \multicolumn{1}{c}{LPIPS$\downarrow$}\\
\midrule
\multirow{3}{*}{MobileNeRF} & Stage 1 & 23.18 & 0.823 & 0.350 \\ 
~ & Stage 2 & 22.10 & 0.784 & 0.412 \\ 
~ & Stage 3 & 20.80 & 0.752 & 0.445 \\ 
\midrule
\multicolumn{2}{c}{Ours} & \textbf{23.41} & \textbf{0.846} & \textbf{0.305} \\ 
\bottomrule
\end{tabular}
}}
\end{table}

==> supple_table/dataset_kitti.tex <==
\begin{table}[t]
\centering
% \fontsize{8}{8}\selectfont
\footnotesize
\setlength\tabcolsep{4pt} 
\renewcommand\arraystretch{1.15}
% \caption{Comparison with other competitive methods on KITTI-360 dataset. }
% \caption{Performance comparison of novel view synthesis with other competitive baselines on \texttt{seq\_1}-\texttt{seq\_5} of KITTI-360 dataset.}
\caption{Details of KITTI-360 dataset.}
% \resizebox{\linewidth}{!}
\setlength{\tabcolsep}{7.8mm}{
{
\begin{tabular}{l c c }
\toprule
Sequence & First frame & Last frame\\
\midrule
\texttt{seq\_1} & 715 & 794 \\
\texttt{seq\_2} & 880 & 959 \\
\texttt{seq\_3} & 1102 & 1181 \\
\texttt{seq\_4} & 2170 & 2249 \\
\texttt{seq\_5} & 2900 & 2979 \\
% \rowcolor{Gray}                  
\bottomrule
\end{tabular}
}}
\label{tab:dataset_kitti}
\end{table}

==> supple_table/dataset_waymo.tex <==
\begin{table*}[htbp]
\centering
% \fontsize{8}{8}\selectfont
\footnotesize
\setlength\tabcolsep{4pt} 
\renewcommand\arraystretch{1.15}
\caption{Details of Waymo dataset.}
% \resizebox{\linewidth}{!}
{
\begin{tabular}{l l c c }
\toprule
Set &  Segment Name/ID & First frame & Last frame\\
\midrule
validation 0000 &  segment-10247954040621004675\_2180\_000\_2200\_000\_with\_camera\_labels & 0 & 80 \\
validation 0000 & segment-1071392229495085036\_1844\_790\_1864\_790\_with\_camera\_labels & 135 & 197 \\
validation 0000 &  segment-11037651371539287009\_77\_670\_97\_670\_with\_camera\_labels & 0 & 164 \\
validation 0001 & segment-13469905891836363794\_4429\_660\_4449\_660\_with\_camera\_labels & 0 & 197 \\
validation 0002 & segment-14333744981238305769\_5658\_260\_5678\_260\_with\_camera\_labels & 0 & 198 \\
validation 0002 & segment-14663356589561275673\_935\_195\_955\_195\_with\_camera\_labels & 0 & 197 \\
% \rowcolor{Gray}                  
\bottomrule
\end{tabular}
}
\label{tab:dataset_waymo}
\end{table*}

==> supple_table/kitti360_comparison_w_depth.tex <==
\begin{table}[t]
\centering
% \fontsize{8}{8}\selectfont
\setlength\tabcolsep{4pt} 
\renewcommand\arraystretch{1.15}
\footnotesize
% \caption{Comparison with other competitive methods on KITTI-360 dataset. }
% \caption{Performance comparison of novel view synthesis with other competitive baselines on \texttt{seq\_1}-\texttt{seq\_5} of KITTI-360 dataset.}
\caption{Performance comparison of novel view synthesis with other competitive baselines on KITTI-360 dataset. $^\dag$ means the method is trained with additional depth supervision.}
% \resizebox{\linewidth}{!}
% {
\begin{tabular}{l c c c}
\toprule
\textbf{Method} & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\midrule
Mip-NeRF$^\dag$~\cite{barron2021mip} & 23.26 & 0.815 & 0.404 \\
Mip-NeRF 360$^\dag$~\cite{barron2022mip} & \textbf{23.43} & 0.837 & 0.354 \\
\midrule
Ours & \underline{23.41} & \textbf{0.846} & \textbf{0.305} \\
% Ours (Pruned) & 23.27 & \underline{0.842} & \underline{0.307} \\
\bottomrule
\end{tabular}
% }
\label{tab:kitti}
% \vspace{-3ex}
\end{table}

==> supple_table/waymo_comparison_w_depth.tex <==
\begin{table}[t]
\centering
% \fontsize{8}{8}\selectfont
\setlength\tabcolsep{4pt} 
\renewcommand\arraystretch{1.15}
% \caption{Comparison with other competitive methods on Waymo Open dataset. }
\caption{
% Quantitative comparison of novel view interpolation on Waymo dataset.
Performance comparison of novel view synthesis with other competitive baselines on  Waymo dataset. $^\dag$ means the method is trained with additional depth supervision.
}
\footnotesize
\begin{tabular}{l c c c}
\toprule
\textbf{Method} & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
\midrule
Mip-NeRF$^\dag$~\cite{barron2021mip} & 27.02 & 0.881 & 0.449 \\
Mip-NeRF 360$^\dag$~\cite{barron2022mip} & 27.46 & \textbf{0.895} & 0.393 \\
\midrule
Ours & \textbf{27.62} & \underline{0.892} & \textbf{0.381} \\
% \midrule
% PSNR$\uparrow$ & 26.24 & 26.92 &   26.26 & 25.62   & 26.96 & \textbf{27.62} \\  
% SSIM$\uparrow$ & 0.870 & 0.885 &     0.868 &  0.879  & 0.880 & \textbf{0.892} \\ 
% LPIPS$\downarrow$ & 0.472 & 0.418   & 0.450 & 0.518   & 0.451 & \textbf{0.381} \\ 
% \rowcolor{Gray}                  
\bottomrule
\end{tabular}
\label{tab:waymo}
% \vspace{-3ex}
\end{table}
